Evaluating Deep Neural Networks in Deployment (A Comparative and Replicability Study)

As deep neural networks (DNNs) are increasingly used in safety-critical applications, there is a growing concern for their reliability. Even highly trained, high-performant networks are not 100% accurate. However, it is very difficult to predict their behavior during deployment without ground truth. In this paper, we provide a comparative and replicability study on recent approaches that have been proposed to evaluate the reliability of DNNs in deployment. We find that it is hard to run and reproduce the results for these approaches on their replication packages and even more difficult to run them on artifacts other than their own. Further, it is difficult to compare the effectiveness of the approaches, due to the lack of clearly defined evaluation metrics. Our results indicate that more effort is needed in our research community to obtain sound techniques for evaluating the reliability of neural networks in safety-critical domains. To this end, we contribute an evaluation framework that incorporates the considered approaches and enables evaluation on common benchmarks, using common metrics.

==> sections/approaches/other_approaches.tex <==

DNN models, specifically classifiers, produce a confidence score for their predictions based on softmax probabilities~\cite{HendrycksG16c}, however metrics such as these and information theory metrics such as entropy have been shown to be unreliable~\cite{8683359},~\cite{NEURIPS2019_757f843a},~\cite{abs-2003-01289}. Other approaches learn other models such as nearest-neighbor classifiers~\cite{jiang2018trust} to measure the confidence of a given DNN. ConfidNet~\cite{NEURIPS2019_757f843a} builds a ConvNet model to learn the confidence criterion based on the true class probability for failure prediction. However, apart from being not scaleable, the effectiveness of such approaches is heavily dependent on the training dataset composition, which usually has fewer mis-classified instances. Dissector, proposed by Wang et al.~\cite{Wang00M020}, focus on distinguishing inputs representing unexpected conditions from normal inputs. A number of sub-models are trained for this purpose which is a time-consuming process, and previous work ~\cite{Xiao2021SelfCheckingDN} highlights that the approach does not provide a clear design of the threshold for distinguishing inputs. The applicability of the technique is also limited to image-models. Another approach designed for self-driving car models is SelfOracle ~\cite{0001WCT20}. The technique monitors video frames or image sequences to identify unsupported driving scenarios based on the estimated confidence in the model output being lesser than a threshold. The performance of this approach has been evaluated to be limited on other DNN types and scenarios~\cite{Xiao2021SelfCheckingDN}.

{\bf divya will expand on the citations below.}
Another recent work on evaluating reliability of DNNs ~\cite{Ghobrial_2023}

Some related work; survey/comparitive study of techniques evaluating model reliability/runtime assurance.
(i) ~\cite{Kentour2021AnalysisOT}, (ii)Technical report https://apps.dtic.mil/sti/citations/AD1113747, (iii) ~\cite{huang2020survey}


\eduard{should we list some criteria for our selection?}
For the purpose of this replicability study, we considered the approaches that satisfy the following criteria; 
\begin{itemize}
    \item Techniques that have been fully developed, are available as open source tools, are in a state that can be quantitatively evaluated.
    \item Techniques that can be considered state-of-the-art: They have been proposed in the past three years, have considerable citations.
    \item Approaches that claim to have broad applicability but have been evaluated only on specific input domains.
    \item Techniques that have been compared with few or no approaches proposed after them.
\end{itemize}

==> sections/methods/input.tex <==
\subsection{Data Representations}
%\eduard{probably this makes part of the background}
Our focus primarily lies on tabular and image data, as the approaches that we are evaluating in this paper have only studied these representations. \corina{not sure we should discuss these as they seem well known}
%However, it's essential to acknowledge other data representations as well. These include text, time series, graph, and audio data. \eduard{citations}

\textbf{Tabular Data}: Tabular data is structured into rows and columns, resembling a spreadsheet or database table. Each row typically represents an instance or observation, while columns correspond to features or attributes describing those instances. Examples of tabular data include datasets from relational databases, CSV files, or Excel spreadsheets. 
%\eduard{citations} \\

\textbf{Image Data}: Image data represents visual information in pixels arranged in a grid. Each pixel's intensity or color value corresponds to a specific feature, and the arrangement of pixels captures the visual content of an image. Image data is commonly used in object detection, image classification, and segmentation tasks. 
%\eduard{citations}\\

In their original respective studies, DeepInfer is evaluated only on tabular data while SelfChecker is evaluated only on image data. In previous work, Prophecy has been evaluated on both tabular and image data, albeit not specifically for predicting errors in DNN output.

%\eduard{to say that future work should consider more data representations for a more comprehensive evaluation of the techniques}
%While we emphasize tabular and image data due to their prominence in current research, recognizing other data types underscores the importance of comprehensive evaluation across diverse representations.\\

==> tables/comparisons.tex <==
%\begin{table*}
%\caption{Comparison of techniques.}\vspace{-0.3cm}
%\label{tab:techniques_comp}
%\begin{scriptsize}
%\begin{small}
%\begin{tabular}{|c|c|c|c|}\hline
%\multirow{2}{*}{\textbf{Comparison Criteria}}&\multicolumn{3}{c|}{\textbf{Techniques}}\\
%\cline{2-4}
%&{\textbf{SelfChecker}}&{\textbf{DeepInfer}}&{\textbf{Prophecy}}\\
%\hline
%\multirow{1}{*}{\textbf{Inputs}}& {model, train set, val set} & {model, val set}& {model, train set, val set}\\
%\hline

%\textbf{\multirow{3}{*}{Offline Analysis}} & {data-driven (KDE)} & {static-analysis (WP)} & {data-driven (DT)}\\\cline{2-4}
%& {White-box} & {White-box} & {White-box}\\\cline{2-4}
%\textbf{algorithm}& {post-cond: op label} & {post cond: prediction interval} & {post-cond: op label, GT}\\
%\hline
%\textbf{\multirow{3}{*}{Monitor}} &{PDD per layer per class}& {Data pre-conds per input feature} & {Rules for correct/incorrect beh per layer} \\\cline{2-4}
%& {profile in terms of} & {assumptions on input} & {corr/inc logic in terms of}\\
%{\textbf{artifacts}} & {internal layer features} & & {internal layer features}\\
%\hline
%\textbf{\multirow{4}{*}{Inference}} & {layer-vise predictions} & {pre-cond violation}& {layer-vise predictions of} \\
%& {of class on input} & {checks on input} & {model behavior on input} \\ \cline{2-4}
%{\textbf{time}}& {aggregation of} & {no aggregation or voting} & {voting based on} \\
%{\textbf{Checks}}& {layer-vise preds} & & {layer-vise preds} \\
%\hline
%\textbf{\multirow{3}{*}{Output}}  & {alarm on wrong op} & {op is correct/incorrect} & {op is correct/incorrect} \\
%& {no uncertain} & {or uncertain} & {or uncertain} \\ \cline{2-4}
%& {advice for correct op} & {no advice} & {no advice} \\ 
%\hline
%\textbf{\multirow{12}{*}{Features}} & {no abstraction.} & {low latency} & {no abstraction.}\\
%& {signals from multiple layers.} & {no data dependence.} & {signals from multiple layers.} \\
%& &  & {applicable to} \\
%& {advice offered on correct op.} & &  {images and tabular data.}\\
%\hline
% & {high inference time latency.} & {no advice.}& {no advice.}\\
%& {scalability impacted by} & {effectiveness impacted by} & {effectiveness impacted by}\\
%& {\# layers, \# classes.} & {abstraction precision.} & {train data (\# corr vs. \#inc).}\\
%& {effectiveness impacted by} & {does not handle image networks.}  & \\
%& {data representativeness.} & {applicability and scalability} & \\
%& {applicable mainly to} & {dependent on} & \\
%& {image classifiers.} & {architecture, input dimensionality.} & \\
%& {no OOD or adv detection.} & {no OOD or adv detection.} & {no OOD or adv detection.}\\
%\hline
%\end{tabular}
%\end{scriptsize}
%\end{small}
%\vspace{-3mm}
%\end{table*}

==> tables/deepinfer.tex <==
\midsepremove
\begin{table*}[htbp]
    \centering
    \caption{Implying trustworthiness in model prediction for unseen data through preconditions (DeepInfer).}
    \label{table:deepinfer}
    \begin{tabular}{c | c | c c | c c c | c c c c | c c c c c c}
    \toprule
    \headcol
     & & \multicolumn{2}{c|}{\textbf{GT}} & \multicolumn{3}{c|}{\textbf{DeepInfer}} & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{6}{c}{\textbf{Metrics}} \\
    \cmidrule{3-17}
    \headcol
    \multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Model}} & \textit{\#C} & \textit{\#I} & \textit{\#C} & \textit{\#I} & \textit{\#U} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{TPR} & \textit{FPR} & \textit{Precision} & \textit{Recall} & \textit{F1} & \textit{MCC} \\
    \midrule
    \cellcolor{lavender} & \textit{PD1} & 60 & 17 & 53 & 24 & 0 & 4 & 20 & 40 & 13 & 23.53\% & 33.33\% & 16.67\% & 23.53\% & 19.51\% & -0.088 \\
    \rowcol
    \textit{Pima} & \textit{PD2} & 56 & 21 & 77 & 0 & 0 & 0 & 0 & 56 & 21 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% &  - \\
    \cellcolor{lavender} \textit{Diabetes} & \textit{PD3} & 56 & 21 & 42 & 34 & 1 & 9 & 25 & 30 & 12 & 42.86\% & 45.45\% & 26.47\% & 42.86\% & 32.73\% & -0.023 \\
    \mintrow
    \cellcolor{lavender} & \textit{PD4} & 61 & 16 & 14 & 62 & 1 & 16 & 46 & 14 & 0 & 100.0\% & 76.67\% & 25.81\% & 100.0\% & 41.03\% & 0.245 \\
     \midrule
    \cellcolor{lavender} & \textit{HP1} & 122 & 24 & 78 & 62 & 6 & 5 & 57 & 59 & 19 & 20.83\% & 49.14\% & 8.06\% & 20.83\% & 11.63\% & -0.215 \\
    \rowcol
    \cellcolor{lavender} \textit{House} & \textit{HP2} & 125 & 21 & 86 & 59 & 1 & 5 & 54 & 70 & 16 & 23.81\% & 43.55\% & 8.47\% & 23.81\% & 12.5\% & -0.141 \\
    \cellcolor{lavender} \textit{Pricing} & \textit{HP3} & 79 & 67 & 146 & 0 & 0 & 0 & 0 & 79 & 67 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & - \\
    \mintrow
    \cellcolor{lavender} & \textit{HP4} & 123 & 23 & 88 & 58 & 0 & 6 & 52 & 71 & 17 & 26.09\% & 42.28\% & 10.34\% & 26.09\% & 14.81\% & -0.121 \\
    \bottomrule
    \multicolumn{17}{c}{\textit{\#C} - Correct; \textit{\#I} - Incorrect; \textit{\#U} - Uncertain; }\\
    \end{tabular}
\end{table*}
\midsepdefault


==> tables/predictions.tex <==
\midsepremove
\begin{table}[!ht]
    \centering
    \caption{Accuracy comparison between the generated and saved predictions for the BM models in the replications package of DeepInfer.}
    \label{table:predictions}
    \begin{tabular}{|l|l|l|}
    \hline
        \headcol
        & \multicolumn{2}{c|}{\textbf{Accuracy}} \\ 
        \cmidrule{2-3}
        \headcol
        \multirow{-2}{*}{\textbf{Model}} & Predicted & Saved \\
        \toprule
        BM1 & 80.95\% & 50.66\% \\ 
        \rowcol
        BM2 & 81.47\% & 50.38\% \\ 
        BM3 & 51.61\% & 51.61\% \\ 
        \rowcol
        BM4 & 78.59\% & 50.43\% \\ 
        BM5 & 81.95\% & 49.72\% \\ 
        \rowcol
        BM6 & 81.14\% & 50.05\% \\ 
        BM7 & 81.33\% & 50.76\% \\ 
        \rowcol
        BM8 & 81.85\% & 50.8\% \\ 
        BM9 & 81.43\% & 50.0\% \\ 
        \rowcol
        BM10 & 51.61\% & 51.61\% \\ 
        BM11 & 80.67\% & 49.81\% \\ 
        \rowcol
        BM12 & 81.62\% & 50.8\% \\ 
        \bottomrule
    \end{tabular}
\end{table}
\midsepdefault


==> tables/pure.tex <==
\midsepremove
\begin{table*}[htbp]
    \centering
    \caption{Implying trustworthiness in model prediction for unseen data through estimators with pure leaves.}
    \label{table:pure}
    \begin{tabular}{c | c | c c | c c c | c c c c | c c c}
    \toprule
    \headcol
     & & \multicolumn{2}{c|}{\textbf{GT}} & \multicolumn{3}{c|}{\textbf{Prophecy}} & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{3}{c}{\textbf{Metrics}} \\
    \cmidrule{3-14}
    \headcol
    \multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Model}} & \textit{\#C} & \textit{\#I} & \textit{\#C} & \textit{\#I} & \textit{\#U} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{Precision} & \textit{Recall} & \textit{F1} \\
    \midrule
    \mintrow
    \cellcolor{lavender} & \textit{PD1} & 60 & 17 & 57 & 5 & 15 & 47 & 10 & 1 & 4 & 82.46\% & 92.16\% & 87.04\% \\
    \rowcol
    \textit{Pima} & \textit{PD2} & 56 & 21 & 57 & 20 & 0 & 44 & 13 & 8 & 12 & 77.19\% & 78.57\% & 77.88\% \\
    \cellcolor{lavender} \textit{Diabetes} & \textit{PD3} & 56 & 21 & 50 & 25 & 2 & 38 & 12 & 8 & 17 & 76.0\% & 69.09\% & 72.38\% \\
    \rowcol
     & \textit{PD4} & 61 & 16 & 65 & 12 & 0 & 51 & 14 & 2 & 10 & 78.46\% & 83.61\% & 80.95\% \\
     \midrule
    \cellcolor{lavender} & \textit{HP1} & 122 & 24 & 131 & 4 & 11 & 112 & 19 & 3 & 1 & 85.5\% & 99.12\% & 91.8\% \\
    \mintrow
    \cellcolor{lavender} \textit{House} & \textit{HP2} & 125 & 21 & 130 & 7 & 9 & 115 & 15 & 4 & 3 & 88.46\% & 97.46\% & 92.74\% \\
    \cellcolor{lavender} \textit{Pricing} & \textit{HP3} & 79 & 67 & 74 & 72 & 0 & 66 & 8 & 59 & 13 & 89.19\% & 83.54\% & 86.27\% \\
    \rowcol
     & \textit{HP4} & 123 & 23 & 133 & 13 & 0 & 115 & 18 & 5 & 8 & 86.47\% & 93.5\% & 89.84\% \\
    \bottomrule
    \multicolumn{14}{c}{\textit{\#C} - Correct; \textit{\#I} - Incorrect; \textit{\#U} - Uncertain; }\\
    \end{tabular}
\end{table*}
\midsepdefault


==> tables/rq1_old.tex <==
\midsepremove
\begin{table*}[htbp]
    \centering
    \caption{Implying trustworthiness in model prediction for unseen data through estimators.}
    \label{table:rq1}
    \begin{tabular}{c | c | c c | c c c | c c c c | c c c c c c}
    \toprule
    \headcol
     & & \multicolumn{2}{c|}{\textbf{GT}} & \multicolumn{3}{c|}{\textbf{Prophecy}} & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{6}{c}{\textbf{Metrics}} \\
    \cmidrule{3-17}
    \headcol
    \multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Model}} & \textit{\#C} & \textit{\#I} & \textit{\#C} & \textit{\#I} & \textit{\#U} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{TPR} & \textit{FPR} & \textit{Precision} & \textit{Recall} & \textit{F1} & \textit{MCC} \\
    \midrule
    \cellcolor{lavender} & \textit{PD1} & 60 & 17 & 56 & 21 & 16 & 7 & 14 & 46 & 10 & 41.18\% & 23.33\% & 33.33\% & 41.18\% & 36.84\% & 0.166 \\
    \mintrow
    \cellcolor{lavender} \textit{Pima} & \textit{PD2} & 56 & 21 & 57 & 20 & 16 & 8 & 12 & 44 & 13 & 38.1\% & 21.43\% & 40.0\% & 38.1\% & 39.02\% & 0.169 \\
    \cellcolor{lavender} \textit{Diabetes} & \textit{PD3} & 56 & 21 & 48 & 29 & 23 & 10 & 19 & 37 & 11 & 47.62\% & 33.93\% & 34.48\% & 47.62\% & 40.0\% & 0.126 \\
    \rowcol
     & \textit{PD4} & 61 & 16 & 67 & 10 & 0 & 2 & 8 & 53 & 14 & 12.5\% & 13.11\% & 20.0\% & 12.5\% & 15.38\% & -0.007 \\
     \midrule
    \cellcolor{lavender} & \textit{HP1} & 122 & 24 & 132 & 14 & 8 & 5 & 9 & 113 & 19 & 20.83\% & 7.38\% & 35.71\% & 20.83\% & 26.32\% & 0.169 \\
    \rowcol
    \textit{House} & \textit{HP2} & 125 & 21 & 130 & 16 & 9 & 6 & 10 & 115 & 15 & 28.57\% & 8.0\% & 37.5\% & 28.57\% & 32.43\% & 0.231 \\
    \mintrow
    \cellcolor{lavender} \textit{Pricing} & \textit{HP3} & 79 & 67 & 50 & 96 & 27 & 66 & 30 & 49 & 1 & 98.51\% & 37.97\% & 68.75\% & 98.51\% & 80.98\% & 0.636 \\
    \rowcol
     & \textit{HP4} & 123 & 23 & 134 & 12 & 0 & 6 & 6 & 117 & 17 & 26.09\% & 4.88\% & 50.0\% & 26.09\% & 34.29\% & 0.281 \\
    \midrule
    \cellcolor{lavender} & dense & 8045 & 1955 & 9798 & 202 & 0 & 139 & 63 & 7982 & 1816 & 68.81\% & 7.11\% & 12.89\% & 0.178 \\
    \rowcol
     & dense (B) & 8045 & 1955 & 7269 & 2731 & 0 & 1311 & 1420 & 6625 & 644 & 48.0\% & 67.06\% & 55.95\% & 0.44 \\
    \cellcolor{lavender} & dense (C) & 8045 & 1955 & 6538 & 3462 & 0 & 1510 & 1952 & 6093 & 445 & 43.62\% & 77.24\% & 55.75\% & 0.442 \\
    \rowcol
     & ID & 8045 & 1955 & 9791 & 209 & 0 & 145 & 64 & 7981 & 1810 & 69.38\% & 7.42\% & 13.4\% & 0.184 \\
    \cellcolor{lavender} & ID (B) & 8045 & 1955 & 6351 & 3649 & 0 & 1504 & 2145 & 5900 & 451 & 41.22\% & 76.93\% & 53.68\% & 0.414 \\
    \rowcol
    & ID (C) & 8045 & 1955 & 6384 & 3616 & 0 & 1555 & 2061 & 5984 & 400 & 43.0\% & 79.54\% & 55.82\% & 0.445 \\
    \cellcolor{lavender} & DA & 8045 & 1955 & 9726 & 274 & 0 & 195 & 79 & 7966 & 1760 & 71.17\% & 9.97\% & 17.5\% & 0.218 \\
    \mintrow
    \cellcolor{lavender} & DA (B) & 8045 & 1955 & 7557 & 2443 & 0 & 1256 & 1187 & 6858 & 699 & 51.41\% & 64.25\% & 57.12\% & 0.457 \\
    \cellcolor{lavender} & DA (C) & 8045 & 1955 & 6373 & 3627 & 0 & 1569 & 2058 & 5987 & 386 & 43.26\% & 80.26\% & 56.22\% & 0.451 \\
    \rowcol
     & IDA & 8045 & 1955 & 9899 & 101 & 0 & 67 & 34 & 8011 & 1888 & 66.34\% & 3.43\% & 6.52\% & 0.119 \\
    \cellcolor{lavender} & IDA (B) & 8045 & 1955 & 7247 & 2753 & 0 & 1351 & 1402 & 6643 & 604 & 49.07\% & 69.1\% & 57.39\% & 0.459 \\
    \rowcol
     \multirow{-12}{*}{\textit{CIFAR10}} & IDA (C) & 8045 & 1955 & 6543 & 3457 & 0 & 1510 & 1947 & 6098 & 445 & 43.68\% & 77.24\% & 55.8\% & 0.442 \\
    \bottomrule
    \multicolumn{17}{c}{\textit{\#C} - Correct; \textit{\#I} - Incorrect; \textit{\#U} - Uncertain; \textit{B} - Balanced; \textit{C} - Confident; \textit{ID} - Input + Dense Layers;}\\
    \multicolumn{17}{c}{\textit{DA} - Dense + Activation Layers; \textit{IDA} - Input + Dense + Activation Layers}\\
    \end{tabular}
\end{table*}
\midsepdefault


==> tables/rq2_old.tex <==
\midsepremove
\begin{table*}[htbp]
    \centering
    \caption{Implying trustworthiness in model prediction for unseen data through pure rules.}
    \label{table:rq2}
    \begin{tabular}{c | c | c c | c c c | c c c c | c c c c c c}
    \toprule
    \headcol
     & & \multicolumn{2}{c|}{\textbf{GT}} & \multicolumn{3}{c|}{\textbf{Prophecy}} & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{6}{c}{\textbf{Metrics}} \\
    \cmidrule{3-17}
    \headcol
    \multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Model}} & \textit{\#C} & \textit{\#I} & \textit{\#C} & \textit{\#I} & \textit{\#U} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{TPR} & \textit{FPR} & \textit{Precision} & \textit{Recall} & \textit{F1} & \textit{MCC} \\
    \midrule
    \mintrow
    \cellcolor{lavender} & \textit{PD1} & 60 & 17 & 40 & 37 & 27 & 12 & 25 & 35 & 5 & 70.59\% & 41.67\% & 32.43\% & 70.59\% & 44.44\% & 0.24
 \\
    \rowcol
    \textit{Pima} & \textit{PD2} & 56 & 21 & 50 & 27 & 0 & 9 & 18 & 38 & 12 & 42.86\% & 32.14\% & 33.33\% & 42.86\% & 37.5\% & 0.1\% \\
    \cellcolor{lavender} \textit{Diabetes} & \textit{PD3} & 56 & 21 & 66 & 11 & 2 & 4 & 7 & 49 & 17 & 19.05\% & 12.5\% & 36.36\% & 19.05\% & 25.0\% & 0.083 \\
    \rowcol
     & \textit{PD4} & 61 & 16 & 55 & 22 & 2 & 4 & 18 & 43 & 12 & 25.0\% & 29.51\% & 18.18\% & 25.0\% & 21.05\% & -0.04 \\
     \midrule
    \cellcolor{lavender} & \textit{HP1} & 122 & 24 & 120 & 26 & 18 & 9 & 17 & 105 & 15 & 37.5\% & 13.93\% & 34.62\% & 37.5\% & 36.0\% & 0.228 \\
    \rowcol
    \cellcolor{lavender} \textit{House} & \textit{HP2} & 125 & 21 & 133 & 13 & 10 & 5 & 8 & 117 & 16 &  23.81\% & 6.4\% & 38.46\% & 23.81\% & 29.41\% & 0.215\ \\
    \mintrow
    \cellcolor{lavender} \textit{Pricing} & \textit{HP3} & 79 & 67 & 82 & 64 & 0 & 51 & 13 & 66 & 16 & 76.12\% & 16.46\% & 79.69\% & 76.12\% & 77.86\% & 0.599 \\
    \rowcol
    & \textit{HP4} & 123 & 23 & 138 & 8 & 0 & 4 & 4 & 119 & 19 & 17.39\% & 3.25\% & 50.0\% & 17.39\% & 25.81\% & 0.226 \\
    \midrule
    \cellcolor{lavender} & DALE f1=0 & 8045 & 1955 & 9722 & 278 & 0 & 191 & 87 & 7958 & 1764 & 9.77 & 1.08\% & 68.71\% & 9.77\% & 17.11\% & 0.21 \\
    \rowcol
    \cellcolor{lavender} & DALE f1=10\% & 8045 & 1955 & 8473 & 1527 & 0 & 845 & 682 & 7363 & 1110 & 43.22\% & 8.48\% & 55.34\% & 43.22\% & 48.54\% & 0.383 \\
    \cellcolor{lavender} & DALE f1=50\% & 8045 & 1955 & 4668 & 5332 & 0 & 1605 & 3727 & 4318 & 350 & 82.1\% & 46.33\% & 30.1\% & 82.1\% & 44.05\% & 0.284 \\
    \mintrow
    \cellcolor{lavender} & DALB f1=0 & 8045 & 1955 & 7237 & 2763 & 0 & 1359 & 1404 & 6641 & 596 & 69.51\% & 17.45\% & 49.19\% & 69.51\% & 57.61\% & 0.462 \\
    \cellcolor{lavender} & DALB f1=10\% & 8045 & 1955 & 7241 & 2759 & 0 & 1336 & 1423 & 6622 & 619 & & & 48.42\% & 68.34\% & 56.68\% & 0.449 \\
    \rowcol
    \multirow{-6}{*}{\textit{CIFAR10}} & DALB f1=50\% & 8045 & 1955 & 4397 & 5603 & 0 & 1770 & 3833 & 4212 & 185 & & & 31.59\% & 90.54\% & 46.84\% & 0.343 \\
    \bottomrule
    \multicolumn{17}{c}{\textit{\#C} - Correct; \textit{\#I} - Incorrect; \textit{\#U} - Uncertain; \textit{DALB} - Dense + Activation Layers on Balanced data}\\
    \multicolumn{17}{c}{\textit{DALE} - Dense + Activation Layers on Entire data}\\
    \end{tabular}
\end{table*}
\midsepdefault


==> tables/selfchecker_old.tex <==
\midsepremove
\begin{table*}[htbp]
    \centering
    \caption{Implying trustworthiness in model prediction for unseen data through preconditions (SelfChecker).}
    \label{table:deepinfer}
    \begin{tabular}{c | c | c c | c c c | c c c c | c c c c c c}
    \toprule
    \headcol
     & & \multicolumn{2}{c|}{\textbf{GT}} & \multicolumn{3}{c|}{\textbf{SelfChecker}} & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{6}{c}{\textbf{Metrics}} \\
    \cmidrule{3-17}
    \headcol
    \multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Model}} & \textit{\#C} & \textit{\#I} & \textit{\#C} & \textit{\#I} & \textit{\#U} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{TPR} & \textit{FPR} & \textit{Precision} & \textit{Recall} & \textit{F1} & \textit{MCC} \\
    \midrule
    \cellcolor{lavender} & \textit{PD1} &  &  &  &  &  & 7 & 5 & 51 & 14 & 33.33\% & 8.93\% & & & 42.42\% & - \\
    \rowcol
    \textit{Pima} & \textit{PD2} &  &  &  &  &  & 3 & 2 & 54 & 18 & 14.29\% & 3.57\% & & & 23.07\% &  - \\
    \cellcolor{lavender} \textit{Diabetes} & \textit{PD3} &  &  &  &  &  & 11 & 13 & 43 & 10 & 52.38\% & 23.21\% & & & 48.89\% & - \\
    \mintrow
    \cellcolor{lavender} & \textit{PD4} & &  &  &  &  & 8 & 3 & 53 & 13 & 38.09\% & 5.36\% & &  & 50.0\% & - \\
     \midrule
    \cellcolor{lavender} & \textit{HP1} &  &  &  &  &  & 58 & 17 & 62 & 9 & 86.57\% & 21.52\% & & & 81.69\% &  - \\
    \rowcol
    \cellcolor{lavender} \textit{House} & \textit{HP2} &  &  &  &  &  & 59 & 12 & 67 & 8 & 88.06\% & 15.19\% & & & 85.51\% &  - \\
    \cellcolor{lavender} \textit{Pricing} & \textit{HP3} &  &  &  &  &  & 57 & 16 & 63 & 10 & 85.07\% & 20.25\% & & & 81.43\% & - \\
    \mintrow
    \cellcolor{lavender} & \textit{HP4} &  &  &  &  &  & 61 & 14 & 65 & 6 & 91.04\% & 17.72\% & & & 85.92\% & - \\
    \bottomrule
    \multicolumn{17}{c}{\textit{\#C} - Correct; \textit{\#I} - Incorrect; \textit{\#U} - Uncertain; }\\
    \end{tabular}
\end{table*}
\midsepdefault


==> tables/tables5_6.tex <==
\midsepremove
\begin{table}
   \centering
    \begin{scriptsize}
    \caption{Effectiveness results by model for SelfChecker.}
    \label{table:rq3_tabular_SC}
    \begin{tabular}{|c|r r r r | r r r r r| |r r r | r r r r | r r r r r|}
    \hline
        \headcol
        & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{5}{c|}{\textbf{Metrics}} \multicolumn{3}{c|}{\textbf{Notifications}} & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{5}{c|}{\textbf{Metrics}} \\
        \cmidrule{2-5}
        \cmidrule{6-10}
        \cmidrule{10-13}
        \cmidrule{14-17}
        \cmidrule{18-22}
        \headcol
        \multirow{-2}{*}{\textbf{Model}} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{TPR} & \textit{FPR} & \textit{Prec.} & \textit{F1} & \textit{MCC} \\ 
        \toprule
        BM1 & 538 & 444 & 76 & 0 & 100\% & 85.38\% & 54.79\% & 70.79\% & 0.283 \\ \rowcol
        BM2 & 536 & 457 & 63 & 2 & 99.63\% & 87.88\% & 53.98\% & 70.02\% & 0.244 \\ 
        BM3 & 534 & 397 & 123 & 4 & 99.26\% & 76.35\% & 57.36\% & 72.7\% & 0.352 \\ \rowcol
        BM4 & 535 & 424 & 96 & 3 & 99.44\% & 81.54\% & 55.79\% & 71.48\% & 0.307 \\ 
        BM5 & 537 & 454 & 66 & 1 & 99.81\% & 87.31\% & 54.19\% & 70.24\% & 0.257 \\ \rowcol
        BM6 & 535 & 450 & 70 & 3 & 99.44\% & 86.54\% & 54.31\% & 70.26\% & 0.255 \\ 
        BM7 & 531 & 372 & 148 & 7 & 98.7\% & 71.54\% & 58.8\% & 73.7\% & 0.384 \\ \rowcol
        BM8 & 535 & 420 & 100 & 3 & 99.44\% & 80.77\% & 56.02\% & 71.67\% & 0.315 \\ 
        BM9 & 534 & 373 & 147 & 4 & 99.26\% & 71.73\% & 58.88\% & 73.91\% & 0.393 \\ \rowcol
        BM10 & 248 & 28 & 492 & 290 & 46.1\% & 5.38\% & 89.86\% & 60.93\% & 0.464 \\ 
        BM11 & 538 & 520 & 0 & 0 & 100.0\% & 100.0\% & 50.85\% & 67.42\% & 0.0 \\ \rowcol
        BM12 & 534 & 397 & 123 & 4 & 99.26\% & 76.35\% & 57.36\% & 72.7\% & 0.352 \\ \midrule
        CIF10 & 1244 & 207 & 7838 & 711 & 63.63\% & 2.57\% & 85.73\% & 73.05\% & 0.688 \\ \midrule
        \rowcol
        GC1 & 0 & 10 & 57 & 33 & 0.0\% & 14.93\% & 0.0\% & 0.0\% & -0.234 \\ 
        GC2 & 19 & 17 & 50 & 14 & 57.58\% & 25.37\% & 52.78\% & 55.07\% & 0.315 \\ \rowcol
        GC3 & 22 & 34 & 33 & 11 & 66.67\% & 50.75\% & 39.29\% & 49.44\% & 0.151 \\ 
        GC4 & 17 & 31 & 36 & 16 & 51.52\% & 46.27\% & 35.42\% & 41.98\% & 0.049 \\ \rowcol
        GC5 & 20 & 17 & 50 & 13 & 60.61\% & 25.37\% & 54.05\% & 57.14\% & 0.343 \\
        GC6 & 12 & 12 & 55 & 21 & 36.36\% & 17.91\% & 50.0\% & 42.11\% & 0.203 \\ 
        \rowcol
        GC7 & 13 & 14 & 53 & 20 & 39.39\% & 20.9\% & 48.15\% & 43.33\% & 0.196 \\ 
        GC8 & 13 & 11 & 56 & 20 & 39.39\% & 16.42\% & 54.17\% & 45.61\% & 0.253 \\
        \rowcol
        GC9 & 17 & 12 & 55 & 16 & 51.52\% & 17.91\% & 58.62\% & 54.84\% & 0.348 \\
        \midrule
        HP1 & 72 & 66 & 8 & 0 & 100.0\% & 89.19\% & 52.17\% & 68.57\% & 0.237 \\
        \rowcol
        HP2 & 60 & 9 & 65 & 12 & 83.33\% & 12.16\% & 86.96\% & 85.11\% & 0.713 \\ 
        HP3 & 58 & 8 & 66 & 14 & 80.56\% & 10.81\% & 87.88\% & 84.06\% & 0.701 \\ 
        \rowcol
        HP4 & 62 & 10 & 64 & 10 & 86.11\% & 13.51\% & 86.11\% & 86.11\% & 0.726 \\ 
        \midrule
        PD1 & 26 & 8 & 37 & 6 & 81.25\% & 17.78\% & 76.47\% & 78.79\% & 0.63 \\ 
        \rowcol
        PD2 & 11 & 5 & 40 & 21 & 34.38\% & 11.11\% & 68.75\% & 45.83\% & 0.283 \\
        PD3 & 29 & 28 & 17 & 3 & 90.62\% & 62.22\% & 50.88\% & 65.17\% & 0.319 \\ 
        \rowcol
        PD4 & 24 & 6 & 39 & 8 & 75.0\% & 13.33\% & 80.0\% & 77.42\% & 0.623 \\ 
        \bottomrule
    \end{tabular}
     \end{scriptsize}
\end{table}

\begin{table}
    \centering
    \begin{scriptsize}
    \caption{Effectiveness results by model for DeepInfer.}
    \label{table:rq3_tabular_DI}
    \begin{tabular}{|r r r | r r r r | r r r r r|}
    \hline
        \headcol
        \multicolumn{3}{c|}{\textbf{Notifications}} & \multicolumn{4}{c|}{\textbf{Confusion Matrix}} & \multicolumn{5}{c|}{\textbf{Metrics}} \\
        \cmidrule{1-3}
        \cmidrule{4-7}
        \cmidrule{8-12}
        \headcol
        \textit{\#C} & \textit{\#I} & \textit{\#U} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{TPR} & \textit{FPR} & \textit{Prec.} & \textit{F1} & \textit{MCC} \\ 
        \toprule
        310 & 748 & 0 & 597 & 151 & 259 & 51 & 92.13\% & 36.83\% & 79.81\% & 85.53\% & 0.592 \\ \rowcol
        753 & 305 & 0 & 246 & 59 & 617 & 136 & 64.4\% & 8.73\% & 80.66\% & 71.62\% & 0.59 \\
        360 & 698 & 0 & 560 & 138 & 290 & 70 & 88.89\% & 32.24\% & 80.23\% & 84.34\% & 0.587 \\ \rowcol
        543 & 515 & 0 & 422 & 93 & 424 & 119 & 78.0\% & 17.99\% & 81.94\% & 79.92\% & 0.6 \\
        506 & 552 & 0 & 427 & 125 & 429 & 77 & 84.72\% & 22.56\% & 77.36\% & 80.87\% & 0.621 \\ \rowcol
        301 & 757 & 0 & 611 & 146 & 243 & 58 & 91.33\% & 37.53\% & 80.71\% & 85.69\% & 0.575 \\ 
        699 & 359 & 0 & 288 & 71 & 573 & 126 & 69.57\% & 11.02\% & 80.22\% & 74.51\% & 0.603 \\ \rowcol
        540 & 518 & 0 & 428 & 90 & 440 & 100 & 81.06\% & 16.98\% & 82.63\% & 81.84\% & 0.641 \\ 
        1058 & 0 & 0 & 0 & 0 & 857 & 201 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0 \\
        \rowcol
        549 & 509 & 0 & 260 & 249 & 260 & 289 & 47.36\% & 48.92\% & 51.08\% & 49.15\% & -0.016 \\ 
        445 & 613 & 0 & 321 & 292 & 199 & 246 & 56.61\% & 59.47\% & 52.37\% & 54.41\% & -0.029 \\ \rowcol
        535 & 523 & 0 & 424 & 99 & 445 & 90 & 82.49\% & 18.2\% & 81.07\% & 81.77\% & 0.643 \\ \midrule
        4570 & 5430 & 0 & 3938 & 1492 & 4107 & 463 & 89.48\% & 26.65\% & 72.52\% & 80.11\% & 0.626 \\
        \midrule
        \rowcol
        52 & 48 & 0 & 30 & 18 & 37 & 15 & 66.67\% & 32.73\% & 62.5\% & 64.52\% & 0.338 \\
        21 & 79 & 0 & 53 & 26 & 14 & 7 & 88.33\% & 65.0\% & 67.09\% & 76.26\% & 0.281 \\
        \rowcol
        74 & 26 & 0 & 16 & 10 & 51 & 23 & 41.03\% & 16.39\% & 61.54\% & 49.23\% & 0.274 \\ 
        56 & 44 & 0 & 38 & 6 & 29 & 27 & 58.46\% & 17.14\% & 86.36\% & 69.72\% & 0.397 \\ 
        \rowcol
        68 & 32 & 0 & 23 & 9 & 44 & 24 & 48.94\% & 16.98\% & 71.88\% & 58.23\% & 0.342 \\
        52 & 48 & 0 & 40 & 8 & 27 & 25 & 61.54\% & 22.86\% & 83.33\% & 70.8\% & 0.369 \\
        \rowcol
        29 & 71 & 0 & 50 & 21 & 17 & 12 & 80.65\% & 55.26\% & 70.42\% & 75.19\% & 0.272 \\ 
        64 & 36 & 0 & 33 & 3 & 34 & 30 & 52.38\% & 8.11\% & 91.67\% & 66.67\% & 0.445 \\
        \rowcol
        41 & 59 & 0 & 45 & 14 & 22 & 19 & 70.31\% & 38.89\% & 76.27\% & 73.17\% & 0.307 \\ \midrule
        77 & 68 & 1 & 64 & 5 & 60 & 17 & 79.01\% & 7.69\% & 92.75\% & 85.33\% & 0.71 \\
        \rowcol
        82 & 64 & 0 & 56 & 8 & 66 & 16 & 77.78\% & 10.81\% & 87.5\% & 82.35\% & 0.675 \\
        146 & 0 & 0 & 0 & 0 & 74 & 72 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0 \\ 
        \rowcol
        78 & 68 & 0 & 60 & 8 & 68 & 10 & 85.71\% & 10.53\% & 88.24\% & 86.96\% & 0.753 \\ 
        \midrule
        53 & 22 & 2 & 21 & 3 & 40 & 13 & 61.76\% & 6.98\% & 87.5\% & 72.41\% & 0.587 \\
        \rowcol
        77 & 0 & 0 & 0 & 0 & 45 & 32 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0 \\ 
        41 & 36 & 0 & 19 & 17 & 27 & 14 & 57.58\% & 38.64\% & 52.78\% & 55.07\% & 0.188 \\ \rowcol
        20 & 57 & 0 & 45 & 12 & 17 & 3 & 93.75\% & 41.38\% & 78.95\% & 85.71\% & 0.579 \\
        \bottomrule
    \end{tabular}
    \end{scriptsize}
\end{table}

